Evaluating Input Perturbation Methods for Interpreting CNNs and Saliency Map Comparison

Input perturbation methods occlude parts of an input to a function and measure the change in the function's output. Recently, input perturbation methods have been applied to generate and evaluate saliency maps from convolutional neural networks. In practice, neutral baseline images are used for the occlusion, such that the baseline image's impact on the classification probability is minimal. However, in this paper we show that arguably neutral baseline images still impact the generated saliency maps and their evaluation with input perturbations. We also demonstrate that many choices of hyperparameters lead to the divergence of saliency maps generated by input perturbations. We experimentally reveal inconsistencies among a selection of input perturbation methods and find that they lack robustness for generating saliency maps and for evaluating saliency maps as saliency metrics.

==> chapters/motivation.tex <==
\section{Motivation}

% \input{chapters/neutral_inputs.tex}

% \input{chapters/novelty_detection.tex}

% \input{chapters/variation.tex}

\section{Variation of Input Perturbations}

\subsection{Variation of Baselines}

Since the choice of the baseline has been arbitrary in the past, we analyze the impact of using different supposedly uninformative baselines for different input perturbation methods.  

Maybe calculate L2-distance between heatmaps? Have some quantative measure for similarity of heatmaps. 

Sliding window. For the sliding window we are using a square with size $33 \mathrm{px} \times 33 \mathrm{px}$, which is comparable to the size used in \cite{zeiler_fergus_2014}. We then move the square to every pixel position, which are $224 \cdot 224 = 50176$ positions. Note that the full square is not visible in the corners or close to the edges. 

% \begin{figure*}[htp!]
% \begin{center}
%     \subfloat[Black baseline]{{\includegraphics[width=0.16\linewidth]{images/variation/sliding_window/sliding_goldfish_0_goldfish_black.jpg}}}%
%     % \qquad
%     \hspace{0.1em}
%     \subfloat[Gray baseline]{{\includegraphics[width=0.16\linewidth]{images/variation/sliding_window/sliding_goldfish_0_goldfish_gray.jpg}}}%
%     % \quadd
%     \hspace{0.1em}
%     \subfloat[White baseline]{{\includegraphics[width=0.16\linewidth]{images/variation/sliding_window/sliding_goldfish_0_goldfish_white.jpg}}}%
%     % \qquad
%     \hspace{0.1em}
%     \subfloat[Mean baseline]{{\includegraphics[width=0.16\linewidth]{images/variation/sliding_window/sliding_goldfish_0_goldfish_mean.jpg}}}%
%     % \qquad
%     \hspace{0.1em}
%     \subfloat[Blur baseline]{{\includegraphics[width=0.16\linewidth]{images/variation/sliding_window/sliding_goldfish_0_goldfish_blur.jpg}}}%
%     \hspace{0.1em}
%      \subfloat[Noise baseline]{{\includegraphics[width=0.16\linewidth]{images/variation/sliding_window/sliding_goldfish_0_goldfish_noise.jpg}}}%
% \end{center}
%   \caption{Sliding Window.}
% \label{fig:short}
% \end{figure*}

\begin{figure}[htp!]
\begin{center}
    \subfloat[Black baseline]{{\includegraphics[width=0.32\linewidth]{images/variation/sliding_window/sliding_catdog_0_bull_mastiff_black.jpg}}}%
    \hspace{0.1em}
    \subfloat[Gray baseline]{{\includegraphics[width=0.32\linewidth]{images/variation/sliding_window/sliding_catdog_0_bull_mastiff_gray.jpg}}}%
    \hspace{0.1em}
    \subfloat[White baseline]{{\includegraphics[width=0.32\linewidth]{images/variation/sliding_window/sliding_catdog_0_bull_mastiff_white.jpg}}}%
    
    \subfloat[Mean baseline]{{\includegraphics[width=0.32\linewidth]{images/variation/sliding_window/sliding_catdog_0_bull_mastiff_mean.jpg}}}%
    \hspace{0.1em}
    \subfloat[Blur baseline]{{\includegraphics[width=0.32\linewidth]{images/variation/sliding_window/sliding_catdog_0_bull_mastiff_blur.jpg}}}%
    \hspace{0.1em}
     \subfloat[Noise baseline]{{\includegraphics[width=0.32\linewidth]{images/variation/sliding_window/sliding_catdog_0_bull_mastiff_noise.jpg}}}%
\end{center}
   \caption{Sliding Window.}
\label{fig:short}
\end{figure}

Insertion and deletion

Since the insertion and deletion metrics compare different saliency maps, we choose two different saliency methods: RISE and Grad-CAM \cite{grad_cam}. The saliency maps have been created for the same class. RISE is being used as presented in \cite{Petsiuk2018rise} with a black baseline $\vec{A}_{\mathrm{0}}$, $N = 16384$ masks, unscaled mask size is $h = w = 7$ and $p = 0.5$. The same results apply to the use of any other two different saliency methods. This is just for demonstration purposes. However, if the heatmap is very diffuse, highlights mostly single pixels, the application of insertion and deletion might not work, because of adversarial examples being created. In the case of the noise image, the same noise image is used for every iteration and for both RISE and Grad-CAM for a fair comparison. (Maybe leave out deletion? to save space?)

\begin{figure}[htp!]
\begin{center}
    \subfloat[Grad-CAM]{{\includegraphics[width=0.235\linewidth]{images/variation/insertion_deletion/gcam_ILSVRC2012_val_00000866_wallet.jpg}}}%
    \hspace{0.1em}
    \subfloat[RISE]{{\includegraphics[width=0.235\linewidth]{images/variation/insertion_deletion/rise_ILSVRC2012_val_00000866_893_mean_data_7_24_v0.jpg}}}%
    \hspace{0.1em}
    % \quadd
    \subfloat[Grad-CAM]{{\includegraphics[width=0.235\linewidth]{images/variation/insertion_deletion/gcam_ILSVRC2012_val_00007603_wig.jpg}}}%
    \hspace{0.1em}
    \subfloat[RISE]{{\includegraphics[width=0.235\linewidth]{images/variation/insertion_deletion/rise_ILSVRC2012_val_00007603_903_mean_data_7_24_v0.jpg}}}%
\end{center}
   \caption{RISE with different baselines, with standard parameters, converged and for the maximum class.}
\label{fig:short}
\end{figure}

\begin{figure}[htp!]
\begin{center}
   \input{figures/variation/insertion_deletion/ILSVRC2012_val_00000866_893_insertion_blur_10_6693.tex}
\end{center}
   \caption{Insertion for cat dog image with blur baseline image for the RISE and Grad-CAM saliency map for class boxer.}
\label{fig:resnet_gray}
\end{figure}

\begin{figure}[htp!]
\begin{center}
   \input{figures/variation/insertion_deletion/ILSVRC2012_val_00000866_893_insertion_mean_data_6693.tex}
\end{center}
   \caption{Insertion for cat dog image with blur baseline image for the RISE and Grad-CAM saliency map for class boxer.}
\label{fig:resnet_gray}
\end{figure}

\begin{figure}[htp!]
\begin{center}
   \input{figures/variation/insertion_deletion/catdog_0_242_insertion_noise.tex}
\end{center}
   \caption{Insertion for cat dog image with noise baseline image for the RISE and Grad-CAM saliency map for class boxer.}
\label{fig:resnet_gray}
\end{figure}

Also note how the curve for the same heatmap changes by changing from one baseline to another baseline. 

\begin{figure}[htp!]
\begin{center}
   \input{figures/variation/insertion_deletion/catdog_0_242_deletion_blur_10.tex}
\end{center}
   \caption{Deletion for cat dog image with blur baseline image for the RISE and Grad-CAM saliency map for class boxer.}
\label{fig:resnet_gray}
\end{figure}

\begin{figure}[htp!]
\begin{center}
   \input{figures/variation/insertion_deletion/catdog_0_242_deletion_noise.tex}
\end{center}
   \caption{Deletion for cat dog image with noise baseline image for the RISE and Grad-CAM saliency map for class boxer.}
\label{fig:resnet_gray}
\end{figure}

Integrated gradients

No attribution if the pixel is the same as the baseline, see formula. Also noted by expected gradients paper. Plot positive and negative separately or use diverging heatmap. Running 512 iterations, which is more than the recommended amount of the authors. Also making sure that the sum of integrated gradients is equal to the difference in prediction scores. Report the maximum difference between prediction scores and integrated gradients. Report the prediction scores for the baselines for the maximum class. 

\begin{equation}
    \epsilon(\vec{X}, \vec{A}) = \left| f(\vec{X}) - f(\vec{A}) - \sum_{i = 1}^{n} S_{IG}^{i}(\vec{X}, \vec{A}) \right|
\end{equation}

\begin{figure}[htp!]
\begin{center}
    \subfloat[Black baseline, $f_{\mathrm{0}} = 5.34 \cdot 10^{-5}$, $\epsilon_{\mathrm{0}} =1.25\cdot10^{-3}$.]{{\includegraphics[width=0.32\linewidth]{images/variation/integrated_gradients/ig_catdog_0_bull_mastiff_black.jpg}}}%
    % \qquad
    \hspace{0.1em}
    \subfloat[Gray baseline, $f_{\mathrm{127}} = 1.70 \cdot 10^{-4}$, $\epsilon_{\mathrm{127}} =8.59\cdot10^{-5}$.]{{\includegraphics[width=0.32\linewidth]{images/variation/integrated_gradients/ig_catdog_0_bull_mastiff_gray.jpg}}}%
    % \quadd
    \hspace{0.1em}
    \subfloat[White baseline, $f_{\mathrm{255}} = 2.62 \cdot 10^{-4}$, $\epsilon_{\mathrm{255}} =8.86\cdot10^{-4}$.]{{\includegraphics[width=0.32\linewidth]{images/variation/integrated_gradients/ig_catdog_0_bull_mastiff_white.jpg}}}%

    \subfloat[Mean baseline, $f_{\mathrm{{\overline{\vec{X}}}}} = 1.78 \cdot 10^{-4}$, $\epsilon_{\mathrm{{\overline{\vec{X}}}}} =7.12\cdot10^{-4}$.]{{\includegraphics[width=0.32\linewidth]{images/variation/integrated_gradients/ig_catdog_0_bull_mastiff_mean.jpg}}}%
    % \qquad
    \hspace{0.1em}
    \subfloat[Blur baseline, $f_{\mathrm{\sigma}} = 1.13 \cdot 10^{-4}$, $\epsilon_{\mathrm{\sigma}} =8.84\cdot10^{-4}$.]{{\includegraphics[width=0.32\linewidth]{images/variation/integrated_gradients/ig_catdog_0_bull_mastiff_blur.jpg}}}%
    \hspace{0.1em}
     \subfloat[Noise baseline, $f_{\mathrm{U}} = 8.91 \cdot 10^{-7}$, $\epsilon_{\mathrm{U}} =2.67\cdot10^{-3}$.]{{\includegraphics[width=0.32\linewidth]{images/variation/integrated_gradients/ig_catdog_0_bull_mastiff_noise.jpg}}}%
\end{center}
   \caption{Integrated Gradients. Read up on best way of displaying integrated gradients heatmap from their paper.}
\label{fig:short}
\end{figure}

RISE
% \input{chapters/convergence.tex} 

\begin{figure}[htp!]
\begin{center}
   \input{figures/convergence/catdog/convergence.tex}
\end{center}
   \caption{Convergence cat dog.}
\label{fig:resnet_gray}
\end{figure}

\begin{figure}[htp!]
\begin{center}
    \subfloat[First run]{{\includegraphics[width=0.235\linewidth]{images/convergence/catdog/mask_32767_0.jpg}}}%
    % \qquad
    \hspace{0.1em}
    \subfloat[Second run]{{\includegraphics[width=0.235\linewidth]{images/convergence/catdog/mask_32767_1.jpg}}}%
    % \quadd
    \hspace{0.1em}
    \subfloat[Third Run]{{\includegraphics[width=0.235\linewidth]{images/convergence/catdog/mask_32767_2.jpg}}}%
    \hspace{0.1em}
    \subfloat[Fourth Run]{{\includegraphics[width=0.235\linewidth]{images/convergence/catdog/mask_32767_3.jpg}}}%
\end{center}
   \caption{Convergence check for RISE (catdog image) 32768 masks.}
\label{fig:short}
\end{figure}

\begin{figure}[htp!]
\begin{center}
    \subfloat[First run]{{\includegraphics[width=0.235\linewidth]{images/convergence/goldfish_50/mask_32767_0.jpg}}}%
    % \qquad
    \hspace{0.1em}
    \subfloat[Second run]{{\includegraphics[width=0.235\linewidth]{images/convergence/goldfish_50/mask_32767_1.jpg}}}%
    % \quadd
    \hspace{0.1em}
    \subfloat[Third Run]{{\includegraphics[width=0.235\linewidth]{images/convergence/goldfish_50/mask_32767_2.jpg}}}%
    \hspace{0.1em}
    \subfloat[Fourth Run]{{\includegraphics[width=0.235\linewidth]{images/convergence/goldfish_50/mask_32767_3.jpg}}}%
\end{center}
   \caption{Convergence check for RISE (goldfish image) 32768 masks, $p = 0.5$.}
\label{fig:short}
\end{figure}

\begin{figure}[htp!]
\begin{center}
    \subfloat[First run]{{\includegraphics[width=0.235\linewidth]{images/convergence/goldfish_10/mask_32767_0.jpg}}}%
    % \qquad
    \hspace{0.1em}
    \subfloat[Second run]{{\includegraphics[width=0.235\linewidth]{images/convergence/goldfish_10/mask_32767_1.jpg}}}%
    % \quadd
    \hspace{0.1em}
    \subfloat[Third Run]{{\includegraphics[width=0.235\linewidth]{images/convergence/goldfish_10/mask_32767_2.jpg}}}%
    \hspace{0.1em}
    \subfloat[Fourth Run]{{\includegraphics[width=0.235\linewidth]{images/convergence/goldfish_10/mask_32767_3.jpg}}}%
\end{center}
   \caption{Convergence check for RISE (goldfish image) 32768 masks, $p = 0.1$.}
\label{fig:short}
\end{figure}

Since there are multiple goldfish in the image, the chance of at least one goldfish being visible is very high. This in return results in a high prediction score. Therefore, the RISE saliency map is not able to converge. In this case we decrease the number of revealed pixels. For example for a $p = 0.1$ the saliency map converges. 

A note on convergence: RISE does not converge in every case. In order to determine convergence and how many masks are needed we run RISE with $p = 0.5$, $h = w = 7$ three times. We then check the similarity between the three heatmaps with their respective L2 distances with every additional mask.
Show case where RISE converges and where it does not converge. In the case RISE does not converge we decrease the parameter $p$, until convergence is reached. 
We choose 16834 masks, which is a good compromise between convergence behavior and computational effort. 

RISE is run with $N = 16384$ masks, by which the saliency map has converged, encourage to check the $\epsilon$ between different saliency maps when adding masks. The small mask size is $h = w = 7$ and $p = 0.5$ (make sure this is actually the case). (Also make sure the same masks have been used for each experiment!). The mask generation follows the approach presented in \cite{Petsiuk2018rise}. 
\begin{figure}[htp!]
\begin{center}
    \subfloat[Mean channelwise]{{\includegraphics[width=0.235\linewidth]{images/variation/rise/rise_ILSVRC2012_val_00021133_24_mean_data_7_24_v0.jpg}}}%
    % \qquad
    \hspace{0.1em}
    \subfloat[White]{{\includegraphics[width=0.235\linewidth]{images/variation/rise/rise_ILSVRC2012_val_00006142_634_white_7_24_v0.jpg}}}%
    % \quadd
    \hspace{0.1em}
    \subfloat[Gray]{{\includegraphics[width=0.235\linewidth]{images/variation/rise/rise_ILSVRC2012_val_00002324_684_gray_7_24_v0.jpg}}}%
    \hspace{0.1em}
    \subfloat[White]{{\includegraphics[width=0.235\linewidth]{images/variation/rise/rise_ILSVRC2012_val_00001218_21_white_7_24_v0.jpg}}}%

    \subfloat[Blur]{{\includegraphics[width=0.235\linewidth]{images/variation/rise/rise_ILSVRC2012_val_00021133_24_blur_7_24_v0.jpg}}}%
    % \qquad
    \hspace{0.1em}
    \subfloat[Black]{{\includegraphics[width=0.235\linewidth]{images/variation/rise/rise_ILSVRC2012_val_00006142_634_black_7_24_v0.jpg}}}%
    \hspace{0.1em}
     \subfloat[Black]{{\includegraphics[width=0.235\linewidth]{images/variation/rise/rise_ILSVRC2012_val_00002324_684_black_7_24_v0.jpg}}}%
     \hspace{0.1em}
    \subfloat[Black]{{\includegraphics[width=0.235\linewidth]{images/variation/rise/rise_ILSVRC2012_val_00001218_21_black_7_24_v0.jpg}}}%
\end{center}
   \caption{RISE with different baselines, with standard parameters, converged and for the maximum class.}
\label{fig:short}
\end{figure}

% \begin{figure}[htp!]
% \begin{center}
%     \subfloat[Black baseline]{{\includegraphics[width=0.32\linewidth]{images/variation/rise/rise_catdog_0_tiger_cat_black.jpg}}}%
%     % \qquad
%     \hspace{0.1em}
%     \subfloat[Gray baseline]{{\includegraphics[width=0.32\linewidth]{images/variation/rise/rise_catdog_0_tiger_cat_gray.jpg}}}%
%     % \quadd
%     \hspace{0.1em}
%     \subfloat[White baseline]{{\includegraphics[width=0.32\linewidth]{images/variation/rise/rise_catdog_0_tiger_cat_white.jpg}}}%

%     \subfloat[Mean baseline]{{\includegraphics[width=0.32\linewidth]{images/variation/rise/rise_catdog_0_tiger_cat_mean.jpg}}}%
%     % \qquad
%     \hspace{0.1em}
%     \subfloat[Blur baseline]{{\includegraphics[width=0.32\linewidth]{images/variation/rise/rise_catdog_0_tiger_cat_blur.jpg}}}%
%     \hspace{0.1em}
%      \subfloat[Noise baseline]{{\includegraphics[width=0.32\linewidth]{images/variation/rise/rise_catdog_0_tiger_cat_noise.jpg}}}%
% \end{center}
%   \caption{RISE for class tiger\_cat.}
% \label{fig:short}
% \end{figure}

Saliency maps with a certain baseline can be misleading. 

\subsection{Variation of Masks}

TODO: Does it make sense to mention? No solution is presented...
Does not apply for integrated gradients and insertion and deletion. Only sliding window and RISE.

Sliding window, \cite{ancn17} have already shown how this approach varies with different square sizes. However, for completeness we attach an example of this as well. Furthermore, we vary the shape we use for occluding. square, circle, equilateral triangle (and rectangle, ellipse?).

RISE variation of $p$. $p \in \{0.1, 0,25, 0.5, 0.75, 0.9\}$, black baseline, $h = w = 7$. Change mask size (greater and smaller $h$ and $w$, but black baseline and $p = 0.5$), smaller sizes might not be able to determine how certain features interact with each other, when they are revealed or occluded. $h = w \in \{5, 7, 9, 11\}$, while $p = 0.5$ (make sure still converges with 16000 masks, since search space increases). 

\begin{figure}[htp!]
\begin{center}
    \subfloat[$p = 0.1$]{{\includegraphics[width=0.32\linewidth]{images/variation/rise/rise_goldfish_0_goldfish_black_7_4.jpg}}}%
    % \qquad
    \hspace{0.1em}
    \subfloat[$p = 0.25$]{{\includegraphics[width=0.32\linewidth]{images/variation/rise/rise_goldfish_0_goldfish_black_7_12.jpg}}}%
    \hspace{0.1em}
    \subfloat[$p = 0.5$]{{\includegraphics[width=0.32\linewidth]{images/variation/rise/rise_goldfish_0_goldfish_black_7_24.jpg}}}%
    % \quadd
    
    \subfloat[$p = 0.75$]{{\includegraphics[width=0.32\linewidth]{images/variation/rise/rise_goldfish_0_goldfish_black_7_36.jpg}}}%
    \hspace{0.1em}
    \subfloat[$p = 0.9$]{{\includegraphics[width=0.32\linewidth]{images/variation/rise/rise_goldfish_0_goldfish_black_7_44.jpg}}}%
\end{center}
   \caption{RISE for class goldfish.}
\label{fig:short}
\end{figure}

\begin{figure}[htp!]
\begin{center}
    \subfloat[$h = w = 5$]{{\includegraphics[width=0.32\linewidth]{images/variation/rise/rise_goldfish_0_goldfish_black_5_12.jpg}}}%
    % \qquad
    \hspace{0.1em}
    \subfloat[$h = w = 7$]{{\includegraphics[width=0.32\linewidth]{images/variation/rise/rise_goldfish_0_goldfish_black_7_24.jpg}}}%
    % \quadd
    
    \subfloat[$h = w = 9$]{{\includegraphics[width=0.32\linewidth]{images/variation/rise/rise_goldfish_0_goldfish_black_9_40.jpg}}}%
    \hspace{0.1em}
    \subfloat[$h = w = 11$]{{\includegraphics[width=0.32\linewidth]{images/variation/rise/rise_goldfish_0_goldfish_black_11_60.jpg}}}%
\end{center}
   \caption{RISE for class goldfish.}
\label{fig:short}
\end{figure}

==> chapters/multiple_baselines.tex <==
\section{Multiple Baselines}

\subsection{Experiments}

==> chapters/neutral_inputs.tex <==
\subsection{Neutral Inputs}

In this section we evaluate, how a DNN classifies a supposedly uninformative input. A neutral input to a DNN contains no class information. Sundararajan \etal define (?) an input $\vec{x} \in \mathbb{R}^n$ to a deep neural network as neutral if ${f(\vec{x}) \approx \vec{0}}$ \cite{Sundararajan2017AxiomaticAF}. However, in the case of a classifier, the last layer is usually a softmax activation function. While the pre-softmax activations for a neutral input are zero, they will be non-zero after the softmax. The softmax for an input with identical elements, \eg ${\vec{x} = \vec{0}}$, is given by $\mathrm{softmax}^{k}(\vec{x}) = {1}/{c}, \forall k \in \{1, ..., c\}$, where $c$ is the number of classes. 

A common choice for a neutral baseline is a black image \cite{Sundararajan2017AxiomaticAF} (and other source for gray image?). Therefore, we choose to record the predictions for all gray images $\mathcal{G} = \{ \{ \gamma \}^{h \times w \times 3} \mid \gamma \in \{0, ..., 255\} \}$, where $\{ 0 \}^{h \times w \times 3}$ is the black image and $\{ 255 \}^{h \times w \times 3}$ is the white image. After appropriate preprocessing they are fed to ResNet50 and we report the maximum predictions for each gray image in  Figure~\ref{fig:resnet_gray}. While each gray image is considered uninformative regarding a class prediction by a human, ResNet50 gives predictions scores, which can be greater than $0.20$ (Although this doesn't really resemble its confidence). Furthermore, for each gray image input there exists at least one ImageNet class with a prediction score greater than $0.05$. This shows that allegedly neutral inputs can have prediction scores greater than ${1}/{c}$ for certain classes, which can consequently not be referred to as neutral. Similar results have been obtained, when running the same experiment with DNNs like VGG-19.

\begin{figure}[htp!]
\begin{center}
   \input{figures/neutral_inputs/resnet_gray_images.tex}
\end{center}
   \caption{Maximum softmax output for different gray image inputs to ResNet50 for a selected number of classes (Somehow can't make the legend transparent and its border disappear).}
\label{fig:resnet_gray}
\end{figure}

(Maybe plot pre-softmax activations instead of softmax output) also plot VGG experiment??

There are three reasons why a DNN's prediction for a supposedly neutral input, specifically the $\vec{x} = \vec{0}$ input or black image in the case of image inputs, does not result in an equal score for each class. First, the bias weights in DNNs are generally nonzero. Even though they might be small, due to penalization during the training process. This leads to nonzero inputs to subsequent layers. (Plot bias weights in ResNet50 and in VGG-19). Second, the pre-processing of the input can transform the input in such a way that the input already becomes nonzero, \eg through mean subtraction/shift. Finally, the training dataset contains biases, such that the DNN associates certain colors with classes. Intuitively, this agrees with human experience such that monitors are often a dark gray color, diswashers a lighter gray and envelopes often white. Similarly, ResNet50 outputs a prediction score of $0.84$ for class jellyfish for a constant blue image with $\vec{x} = \{\left( 0, 0, 255 \right)^{\intercal} \}^{h \times w}$, which supports the argument that ResNet50 has learned certain biases based on the color of an image. (maybe plot a couple of images/calculate mean RGB value of training examples of the different classes in the above plot -- actually there does not seem to be a connection between the mean of a class and the observed behavior. What about plotting a color palette with according classes and scores?).
% \begin{table}[]
%     \begin{center}
%         \begin{tabular}{lll}
%             \toprule
%             Class & $\bar{\vec{x}}_{\mathrm{\{class\}}}$ & $\vec{\sigma}_{\mathrm{\{class\}}}$ \\
%             \midrule
%             envelope & $\left( 0, 0, 255 \right)^{\intercal}$ & $\left( 0, 0, 255 \right)^{\intercal}$\\
%             nematode & $\left( 0, 0, 255 \right)^{\intercal}$ & $\left( 0, 0, 255 \right)^{\intercal}$\\
%             web\_site & $\left( 0, 0, 255 \right)^{\intercal}$ & $\left( 0, 0, 255 \right)^{\intercal}$\\
%             dishwasher & $\left( 0, 0, 255 \right)^{\intercal}$ & $\left( 0, 0, 255 \right)^{\intercal}$\\
%             monitor & $\left( 0, 0, 255 \right)^{\intercal}$ & $\left( 0, 0, 255 \right)^{\intercal}$\\
%             \bottomrule
%         \end{tabular}
%     \end{center}
%     \caption{Mean (or expected value?) and standard deviation for each RGB-channel for the unprocessed training images for different classes}
%     \label{tab:my_label}
% \end{table}

However, assuming there is a neutral input available, \eg generated through an optimization process, then  once this neutral input is used for perturbation methods, we might cover parts of the input which are responsible for canceling out negative or positive activations. Therefore, having to create a neutral input for each mask is not feasible. 

==> chapters/novelty_detection.tex <==
\subsection{Novelty Detection for Perturbed Inputs}

PCA, and parameters

KDE, kernel, parameters. Show most likely images and least likely images maybe in appendix? training and validation data comparison in appendix as well?

Validating our neutral input gray image experiment.
